A Deep Dive into Effects of Structural Bias on CMA-ES Performance along Affine Trajectories

To guide the design of better iterative optimisation heuristics, it is imperative to understand how inherent structural biases within algorithm components affect the performance on a wide variety of search landscapes. This study explores the impact of structural bias in the modular Covariance Matrix Adaptation Evolution Strategy (modCMA), focusing on the roles of various modulars within the algorithm. Through an extensive investigation involving 435,456 configurations of modCMA, we identified key modules that significantly influence structural bias of various classes. Our analysis utilized the Deep-BIAS toolbox for structural bias detection and classification, complemented by SHAP analysis for quantifying module contributions. The performance of these configurations was tested on a sequence of affine-recombined functions, maintaining fixed optimum locations while gradually varying the landscape features. Our results demonstrate an interplay between module-induced structural bias and algorithm performance across different landscape characteristics.

==> cma_bias_newclasses_bounds.tex <==

\begin{tabular}{l|lllllllllllllr}
\toprule
id & active & covariance & elitist & orthogonal & sequential & threshold & sigma & bound_correction & mirrored & base_sampler & weights_option & local_restart & step_size_adaptation & bounds \\
\midrule
16257 & False (0.00) & False (1.00) & True (0.93) & True (0.00) & False (0.00) & True (0.00) & False (0.00) & saturate (0.60) & mirrored (0.00) & halton (0.00) & 1/2^lambda (0.00) & BIPOP (0.00) & tpa (0.00) & 1.000000 \\
161719 & True (0.00) & False (0.60) & True (1.00) & False (0.00) & True (0.00) & True (0.00) & False (0.00) & saturate (0.97) & mirrored (0.00) & sobol (0.00) & 1/2^lambda (0.00) & IPOP (0.00) & msr (0.20) & 1.000000 \\
89773 & True (0.00) & False (0.88) & True (1.00) & False (0.00) & True (0.00) & True (0.00) & False (0.00) & saturate (0.99) & mirrored (0.00) & sobol (0.00) & default (0.00) & IPOP (0.00) & msr (0.33) & 1.000000 \\
89772 & True (0.00) & False (0.94) & True (1.00) & False (0.19) & True (0.00) & False (0.00) & False (0.00) & saturate (0.93) & mirrored (0.00) & sobol (0.00) & 1/2^lambda (0.00) & IPOP (0.00) & msr (0.43) & 1.000000 \\
89771 & True (0.00) & False (1.00) & True (1.00) & False (1.00) & True (0.00) & False (0.00) & False (0.00) & saturate (0.97) & mirrored (0.00) & sobol (0.00) & equal (0.00) & IPOP (0.00) & msr (0.77) & 1.000000 \\
89770 & True (0.00) & False (1.00) & True (1.00) & False (1.00) & True (0.00) & False (0.00) & False (0.00) & saturate (0.99) & mirrored (0.00) & sobol (0.00) & default (0.00) & IPOP (0.00) & msr (0.60) & 1.000000 \\
89769 & True (0.00) & False (1.00) & True (1.00) & False (0.00) & True (0.00) & True (0.00) & False (0.00) & saturate (0.94) & mirrored (0.00) & sobol (0.00) & 1/2^lambda (0.00) & IPOP (0.00) & tpa (0.20) & 1.000000 \\
89765 & True (0.00) & False (1.00) & True (1.00) & False (0.00) & True (0.00) & True (0.00) & False (0.00) & saturate (0.98) & mirrored (0.00) & sobol (0.00) & default (0.00) & IPOP (0.00) & tpa (0.33) & 1.000000 \\
161726 & True (0.00) & False (0.86) & True (1.00) & False (1.00) & True (0.00) & False (0.00) & True (0.00) & saturate (0.98) & nan (0.00) & halton (0.00) & default (0.00) & IPOP (0.00) & msr (0.53) & 1.000000 \\
89762 & True (0.00) & False (1.00) & True (1.00) & False (0.00) & True (0.00) & True (0.00) & True (0.00) & saturate (0.99) & nan (0.00) & halton (0.00) & 1/2^lambda (0.00) & IPOP (0.50) & tpa (0.21) & 1.000000 \\
161723 & True (0.00) & False (1.00) & True (1.00) & False (0.00) & True (0.00) & True (0.00) & True (0.00) & saturate (0.99) & nan (0.00) & halton (0.00) & equal (0.00) & IPOP (0.00) & tpa (0.50) & 1.000000 \\
161722 & True (0.00) & False (1.00) & True (1.00) & False (1.00) & True (0.00) & False (0.00) & False (0.00) & saturate (1.00) & mirrored (0.00) & sobol (0.00) & equal (0.00) & IPOP (0.00) & tpa (0.77) & 1.000000 \\
161721 & True (0.00) & False (1.00) & True (1.00) & False (0.00) & True (0.00) & True (0.00) & True (0.00) & saturate (0.99) & nan (0.00) & halton (0.00) & default (0.00) & IPOP (0.50) & tpa (0.30) & 1.000000 \\
89774 & True (0.00) & False (1.00) & True (1.00) & False (1.00) & True (0.00) & False (0.00) & True (0.00) & saturate (1.00) & nan (0.00) & halton (0.00) & 1/2^lambda (0.00) & IPOP (0.50) & tpa (0.48) & 1.000000 \\
93923 & False (0.97) & True (0.97) & True (0.42) & True (0.08) & False (0.31) & True (0.97) & False (0.03) & saturate (0.92) & nan (0.05) & gaussian (0.07) & 1/2^lambda (0.46) & nan (0.90) & psr (0.69) & x\\ % 14
22019 & False (0.97) & True (0.97) & True (0.64) & True (0.21) & False (0.19) & True (0.97) & False (0.01) & saturate (0.94) & mirrored pairwise (0.04) & sobol (0.05) & 1/2^lambda (0.46) & nan (0.92) & psr (0.63) & x \\ % 18
167136 & False (0.84) & True (0.97) & True (0.83) & False (0.97) & True (0.09) & False (0.10) & True (0.05) & saturate (0.97) & mirrored pairwise (0.07) & halton (0.19) & default (0.30) & nan (0.96) & msr (0.84) & x \\ % 11
21609 & False (0.93) & True (0.97) & True (0.42) & False (0.24) & True (0.15) & True (0.10) & False (0.29) & saturate (0.96) & mirrored (0.16) & sobol (0.21) & default (0.59) & nan (0.97) & msr (0.73) & 0.974452 \\
166529 & False (0.98) & True (0.98) & True (0.05) & True (0.21) & False (0.05) & True (0.98) & True (0.00) & saturate (0.83) & nan (0.10) & halton (0.18) & 1/2^lambda (0.78) & nan (0.90) & lpxnes (0.72) & x \\ % 4
166571 & False (0.98) & True (0.98) & True (0.05) & True (0.21) & False (0.05) & True (0.98) & False (0.00) & saturate (0.83) & nan (0.10) & halton (0.18) & 1/2^lambda (0.78) & nan (0.90) & lpxnes (0.56) & x \\
21641 & False (0.77) & True (0.98) & True (0.77) & False (0.31) & True (0.15) & True (0.09) & True (0.14) & saturate (0.94) & mirrored (0.05) & sobol (0.02) & 1/2^lambda (0.39) & nan (0.59) & psr (0.68) & x \\
94605 & False (0.25) & True (0.98) & True (0.14) & True (0.19) & False (0.52) & True (0.69) & False (0.14) & saturate (0.97) & mirrored pairwise (0.09) & gaussian (0.15) & default (0.35) & nan (0.88) & msr (0.77) & x \\ % 7
\bottomrule
\end{tabular}

==> cma_bias_newclasses_centre.tex <==
\begin{tabular}{l|lllllllllllllr}
\toprule
id & active & covariance & elitist & orthogonal & sequential & threshold & sigma & bound_correction & mirrored & base_sampler & weights_option & local_restart & step_size_adaptation & centre \\
\midrule
392020 & True (0.02) & False (0.02) & True (0.01) & True (0.04) & False (0.04) & True (0.88) & True (0.04) & mirror (0.41) & mirrored pairwise (0.02) & halton (0.02) & equal (0.08) & IPOP (0.04) & mxnes (0.60) & 0.997873 \\
123526 & False (0.04) & False (0.02) & False (1.00) & True (0.07) & False (0.01) & True (0.07) & True (0.02) & toroidal (0.40) & mirrored (0.12) & gaussian (0.01) & equal (0.02) & BIPOP (0.05) & csa (0.12) & 0.997591 \\
424102 & True (0.02) & False (0.05) & False (0.41) & False (0.02) & False (0.01) & True (0.13) & True (0.02) & uniform (0.43) & mirrored pairwise (0.01) & halton (0.02) & equal (0.21) & nan (0.05) & xnes (0.12) & 0.997548 \\
122518 & False (0.04) & False (0.02) & False (0.59) & True (0.11) & False (0.02) & True (0.07) & True (0.02) & toroidal (0.40) & mirrored (0.12) & gaussian (0.01) & equal (0.02) & IPOP (0.05) & csa (0.13) & 0.997508 \\
283909 & True (0.01) & False (0.06) & True (0.87) & True (0.04) & True (0.01) & False (0.09) & True (0.19) & uniform (0.42) & mirrored (0.01) & sobol (0.01) & equal (0.02) & BIPOP (0.26) & mxnes (0.28) & 0.997252 \\
415999 & True (0.02) & False (0.08) & True (0.01) & False (0.87) & False (0.02) & False (0.01) & False (0.00) & toroidal (0.37) & mirrored pairwise (0.02) & halton (0.01) & equal (0.04) & IPOP (0.09) & mxnes (0.33) & 0.997137 \\
258318 & True (0.00) & False (0.03) & True (0.07) & True (0.99) & True (0.01) & False (0.99) & False (0.02) & cotn (0.22) & nan (0.04) & sobol (0.01) & default (0.05) & IPOP (0.78) & msr (0.41) & 0.997078 \\
174006 & False (0.01) & False (0.22) & True (0.05) & True (0.85) & True (0.01) & False (0.82) & True (0.01) & mirror (0.26) & mirrored (0.06) & halton (0.01) & default (0.04) & IPOP (0.77) & csa (0.09) & 0.997077 \\
41263 & False (0.01) & False (0.02) & True (0.03) & True (0.99) & True (0.06) & False (1.00) & False (0.02) & cotn (0.41) & mirrored pairwise (0.02) & sobol (0.02) & equal (0.34) & IPOP (0.97) & msr (0.18) & 0.996977 \\
246364 & True (0.01) & False (0.08) & True (0.01) & False (0.01) & False (0.01) & True (0.01) & True (0.02) & mirror (0.38) & mirrored (0.01) & sobol (0.01) & equal (0.25) & IPOP (0.10) & mxnes (0.62) & 0.996775 \\
210328 & False (0.01) & False (0.00) & True (0.04) & True (0.05) & True (0.01) & True (0.46) & True (0.01) & uniform (0.41) & mirrored (0.04) & halton (0.01) & equal (0.15) & IPOP (0.11) & mxnes (0.59) & 0.996721 \\
53037 & False (0.02) & False (0.02) & True (0.02) & True (0.07) & True (0.01) & True (0.29) & False (0.03) & toroidal (0.44) & mirrored (0.01) & sobol (0.01) & default (0.06) & IPOP (0.32) & mxnes (0.78) & 0.996703 \\
427762 & True (0.01) & False (0.04) & True (0.02) & False (0.03) & False (0.01) & True (0.02) & False (0.02) & uniform (0.39) & mirrored (0.01) & halton (0.01) & equal (0.14) & IPOP (0.12) & mxnes (0.57) & 0.996695 \\
275380 & True (0.07) & True (0.05) & True (0.01) & True (0.10) & False (0.05) & True (0.89) & False (0.00) & toroidal (0.40) & nan (0.01) & sobol (0.01) & equal (0.01) & nan (0.01) & xnes (0.03) & 0.996616 \\
246517 & True (0.01) & False (0.03) & True (0.04) & True (0.90) & False (0.01) & False (0.93) & True (0.02) & mirror (0.38) & mirrored (0.05) & sobol (0.00) & equal (0.18) & IPOP (1.00) & msr (0.44) & 0.996567 \\
258319 & True (0.01) & False (0.08) & True (0.13) & True (0.94) & True (0.05) & False (0.99) & False (0.01) & cotn (0.20) & nan (0.04) & sobol (0.03) & equal (0.05) & IPOP (0.39) & msr (0.51) & 0.996438 \\
114433 & False (0.01) & False (0.24) & True (0.97) & True (0.39) & False (0.01) & False (0.80) & False (0.04) & cotn (0.79) & mirrored (0.46) & gaussian (0.01) & equal (0.22) & BIPOP (0.19) & xnes (0.39) & 0.996413 \\
306000 & True (0.00) & False (0.07) & True (0.14) & True (1.00) & False (0.02) & False (1.00) & True (0.01) & saturate (0.22) & mirrored (0.15) & gaussian (0.01) & default (0.04) & nan (0.70) & mxnes (0.81) & 0.996413 \\
67731 & False (0.01) & True (0.01) & False (0.01) & True (0.23) & False (0.02) & True (0.99) & False (0.10) & uniform (0.40) & nan (0.02) & sobol (0.05) & default (0.06) & IPOP (0.05) & xnes (0.11) & 0.996347 \\
414289 & True (0.09) & False (0.97) & True (0.97) & False (0.97) & False (0.06) & False (0.23) & False (0.03) & toroidal (0.44) & nan (0.03) & halton (0.04) & equal (0.65) & nan (0.97) & csa (0.96) & x \\
\bottomrule
\end{tabular}


==> cma_bias_newclasses_mixed.tex <==


\begin{tabular}{l|lllllllllllllr}
\toprule
id & active & covariance & elitist & orthogonal & sequential & threshold & sigma & bound_correction & mirrored & base_sampler & weights_option & local_restart & step_size_adaptation & bounds \\
\midrule
89768 & True (0.00) & False (1.00) & True (1.00) & False (0.00) & True (0.00) & True (0.00) & True (0.00) & saturate (0.96) & nan (0.00) & halton (0.00) & equal (0.00) & IPOP (0.00) & msr (0.50) & x \\
89767 & True (0.00) & False (0.92) & True (1.00) & False (0.00) & True (0.00) & True (0.00) & True (0.00) & saturate (0.98) & nan (0.00) & halton (0.00) & default (0.00) & IPOP (0.00) & msr (0.30) & x\\
89766 & True (0.00) & False (0.62) & True (1.00) & False (1.00) & True (0.00) & False (0.00) & True (0.00) & saturate (0.97) & nan (0.00) & halton (0.00) & 1/2^lambda (0.00) & IPOP (0.00) & msr (0.48) & x \\
161735 & True (0.00) & False (1.00) & True (1.00) & False (0.00) & True (0.00) & True (0.00) & False (0.00) & saturate (1.00) & mirrored (0.00) & sobol (0.00) & equal (0.00) & IPOP (0.00) & tpa (0.53) & x \\ %10
22782 & False (0.16) & True (1.00) & True (0.03) & True (1.00) & True (0.01) & False (1.00) & False (0.02) & saturate (0.15) & mirrored (0.02) & sobol (0.05) & default (0.29) & IPOP (0.30) & msr (0.50) & x\\
157412 & False (0.42) & False (0.12) & False (0.98) & False (0.94) & True (0.07) & False (0.37) & True (0.00) & saturate (0.88) & nan (0.15) & halton (0.15) & 1/2^lambda (0.98) & nan (0.08) & lpxnes (0.68) & x \\ % 1
157370 & False (0.42) & False (0.12) & False (0.98) & False (0.94) & True (0.07) & False (0.37) & False (0.00) & saturate (0.88) & nan (0.15) & halton (0.15) & 1/2^lambda (0.98) & nan (0.08) & lpxnes (0.61) & x \\
\bottomrule
\end{tabular}

==> cma_bias_newclasses_unif.tex <==
\begin{tabular}{l|lllllllllllllr}
\toprule
id & active & covariance & elitist & orthogonal & sequential & threshold & sigma & bound_correction & mirrored & base_sampler & weights_option & local_restart & step_size_adaptation & unif \\
\midrule
29163 & False (0.05) & False (0.98) & True (0.97) & True (0.06) & True (0.04) & True (0.98) & False (0.07) & mirror (0.50) & mirrored pairwise (0.20) & sobol (0.22) & default (0.30) & IPOP (0.98) & tpa (0.45) & 0.980305 \\
319331 & True (0.04) & False (0.98) & True (0.98) & False (0.29) & True (0.12) & True (0.17) & True (0.14) & mirror (0.50) & mirrored pairwise (0.05) & gaussian (0.07) & 1/2^lambda (0.09) & IPOP (0.98) & csa (0.32) & 0.979526 \\
319341 & True (0.38) & False (0.98) & True (0.98) & False (0.06) & True (0.01) & True (0.09) & True (0.35) & mirror (0.47) & mirrored pairwise (0.04) & gaussian (0.04) & default (0.07) & IPOP (0.98) & tpa (0.38) & 0.976368 \\
269476 & True (0.07) & False (0.98) & True (0.98) & False (0.03) & False (0.04) & True (0.08) & False (0.07) & toroidal (0.43) & mirrored (0.13) & sobol (0.04) & equal (0.73) & nan (0.73) & csa (0.94) & 0.975774 \\
236600 & True (0.53) & True (0.20) & False (0.58) & False (0.25) & False (0.47) & False (0.08) & True (0.13) & saturate (0.94) & mirrored pairwise (0.47) & sobol (0.12) & 1/2^lambda (0.66) & nan (0.31) & tpa (0.44) & 0.974902 \\
100090 & False (0.19) & False (0.97) & True (0.87) & True (0.14) & True (0.07) & True (0.97) & True (0.05) & mirror (0.47) & nan (0.08) & gaussian (0.03) & equal (0.90) & nan (0.60) & csa (0.80) & 0.973789 \\
403005 & True (0.06) & False (0.97) & True (0.97) & False (0.21) & True (0.22) & True (0.15) & True (0.01) & cotn (0.80) & mirrored pairwise (0.13) & halton (0.13) & default (0.28) & nan (0.15) & tpa (0.42) & 0.973032 \\
308705 & True (0.23) & True (0.97) & False (0.97) & True (0.03) & True (0.15) & True (0.97) & False (0.14) & saturate (0.90) & nan (0.10) & gaussian (0.11) & 1/2^lambda (0.22) & nan (0.38) & csa (0.48) & 0.972774 \\
391504 & True (0.07) & False (0.83) & True (0.97) & False (0.08) & False (0.05) & True (0.04) & True (0.03) & mirror (0.44) & mirrored (0.03) & halton (0.15) & equal (0.11) & IPOP (0.97) & msr (0.70) & 0.972369 \\
\bottomrule
\end{tabular}





==> cma_bias_top20_bounds_original20.tex <==
\begin{tabular}{l|lllllllllllllr}
\toprule
id & active & covariance & elitist & orthogonal & sequential & threshold & sigma & bound_correction & mirrored & base_sampler & weights_option & local_restart & step_size_adaptation & bounds \\
\midrule
16257 & False (0.00) & False (1.00) & True (0.93) & True (0.00) & False (0.00) & True (0.00) & False (0.00) & saturate (0.60) & mirrored (0.00) & halton (0.00) & 1/2^lambda (0.00) & BIPOP (0.00) & tpa (0.00) & 1.000000 \\
161719 & True (0.00) & False (0.60) & True (1.00) & False (0.00) & True (0.00) & True (0.00) & False (0.00) & saturate (0.97) & mirrored (0.00) & sobol (0.00) & 1/2^lambda (0.00) & IPOP (0.00) & msr (0.20) & 1.000000 \\
89773 & True (0.00) & False (0.88) & True (1.00) & False (0.00) & True (0.00) & True (0.00) & False (0.00) & saturate (0.99) & mirrored (0.00) & sobol (0.00) & default (0.00) & IPOP (0.00) & msr (0.33) & 1.000000 \\
89772 & True (0.00) & False (0.94) & True (1.00) & False (0.19) & True (0.00) & False (0.00) & False (0.00) & saturate (0.93) & mirrored (0.00) & sobol (0.00) & 1/2^lambda (0.00) & IPOP (0.00) & msr (0.43) & 1.000000 \\
89771 & True (0.00) & False (1.00) & True (1.00) & False (1.00) & True (0.00) & False (0.00) & False (0.00) & saturate (0.97) & mirrored (0.00) & sobol (0.00) & equal (0.00) & IPOP (0.00) & msr (0.77) & 1.000000 \\
89770 & True (0.00) & False (1.00) & True (1.00) & False (1.00) & True (0.00) & False (0.00) & False (0.00) & saturate (0.99) & mirrored (0.00) & sobol (0.00) & default (0.00) & IPOP (0.00) & msr (0.60) & 1.000000 \\
89769 & True (0.00) & False (1.00) & True (1.00) & False (0.00) & True (0.00) & True (0.00) & False (0.00) & saturate (0.94) & mirrored (0.00) & sobol (0.00) & 1/2^lambda (0.00) & IPOP (0.00) & tpa (0.20) & 1.000000 \\
89768 & True (0.00) & False (1.00) & True (1.00) & False (0.00) & True (0.00) & True (0.00) & True (0.00) & saturate (0.96) & nan (0.00) & halton (0.00) & equal (0.00) & IPOP (0.00) & msr (0.50) & 1.000000 \\
89767 & True (0.00) & False (0.92) & True (1.00) & False (0.00) & True (0.00) & True (0.00) & True (0.00) & saturate (0.98) & nan (0.00) & halton (0.00) & default (0.00) & IPOP (0.00) & msr (0.30) & 1.000000 \\
89766 & True (0.00) & False (0.62) & True (1.00) & False (1.00) & True (0.00) & False (0.00) & True (0.00) & saturate (0.97) & nan (0.00) & halton (0.00) & 1/2^lambda (0.00) & IPOP (0.00) & msr (0.48) & 1.000000 \\
161735 & True (0.00) & False (1.00) & True (1.00) & False (0.00) & True (0.00) & True (0.00) & False (0.00) & saturate (1.00) & mirrored (0.00) & sobol (0.00) & equal (0.00) & IPOP (0.00) & tpa (0.53) & 1.000000 \\
89765 & True (0.00) & False (1.00) & True (1.00) & False (0.00) & True (0.00) & True (0.00) & False (0.00) & saturate (0.98) & mirrored (0.00) & sobol (0.00) & default (0.00) & IPOP (0.00) & tpa (0.33) & 1.000000 \\
161728 & True (0.00) & False (1.00) & True (1.00) & False (1.00) & True (0.00) & False (0.00) & True (0.00) & saturate (0.98) & nan (0.00) & halton (0.00) & equal (0.00) & IPOP (0.00) & msr (0.82) & 1.000000 \\
161727 & True (0.00) & False (1.00) & True (1.00) & False (0.88) & True (0.00) & False (0.00) & False (0.00) & saturate (1.00) & mirrored (0.00) & sobol (0.00) & 1/2^lambda (0.00) & IPOP (0.00) & tpa (0.43) & 1.000000 \\
161726 & True (0.00) & False (0.86) & True (1.00) & False (1.00) & True (0.00) & False (0.00) & True (0.00) & saturate (0.98) & nan (0.00) & halton (0.00) & default (0.00) & IPOP (0.00) & msr (0.53) & 1.000000 \\
89762 & True (0.00) & False (1.00) & True (1.00) & False (0.00) & True (0.00) & True (0.00) & True (0.00) & saturate (0.99) & nan (0.00) & halton (0.00) & 1/2^lambda (0.00) & IPOP (0.50) & tpa (0.21) & 1.000000 \\
161723 & True (0.00) & False (1.00) & True (1.00) & False (0.00) & True (0.00) & True (0.00) & True (0.00) & saturate (0.99) & nan (0.00) & halton (0.00) & equal (0.00) & IPOP (0.00) & tpa (0.50) & 1.000000 \\
161722 & True (0.00) & False (1.00) & True (1.00) & False (1.00) & True (0.00) & False (0.00) & False (0.00) & saturate (1.00) & mirrored (0.00) & sobol (0.00) & equal (0.00) & IPOP (0.00) & tpa (0.77) & 1.000000 \\
161721 & True (0.00) & False (1.00) & True (1.00) & False (0.00) & True (0.00) & True (0.00) & True (0.00) & saturate (0.99) & nan (0.00) & halton (0.00) & default (0.00) & IPOP (0.50) & tpa (0.30) & 1.000000 \\
89774 & True (0.00) & False (1.00) & True (1.00) & False (1.00) & True (0.00) & False (0.00) & True (0.00) & saturate (1.00) & nan (0.00) & halton (0.00) & 1/2^lambda (0.00) & IPOP (0.50) & tpa (0.48) & 1.000000 \\
\bottomrule
\end{tabular}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






==> cma_bias_top20_centre_original20.tex <==
\begin{tabular}{l|lllllllllllllr}
\toprule
id & active & covariance & elitist & orthogonal & sequential & threshold & sigma & bound_correction & mirrored & base_sampler & weights_option & local_restart & step_size_adaptation & centre \\
\midrule
392020 & True (0.02) & False (0.02) & True (0.01) & True (0.04) & False (0.04) & True (0.88) & True (0.04) & mirror (0.41) & mirrored pairwise (0.02) & halton (0.02) & equal (0.08) & IPOP (0.04) & mxnes (0.60) & 0.997873 \\
123526 & False (0.04) & False (0.02) & False (1.00) & True (0.07) & False (0.01) & True (0.07) & True (0.02) & toroidal (0.40) & mirrored (0.12) & gaussian (0.01) & equal (0.02) & BIPOP (0.05) & csa (0.12) & 0.997591 \\
424102 & True (0.02) & False (0.05) & False (0.41) & False (0.02) & False (0.01) & True (0.13) & True (0.02) & uniform (0.43) & mirrored pairwise (0.01) & halton (0.02) & equal (0.21) & nan (0.05) & xnes (0.12) & 0.997548 \\
122518 & False (0.04) & False (0.02) & False (0.59) & True (0.11) & False (0.02) & True (0.07) & True (0.02) & toroidal (0.40) & mirrored (0.12) & gaussian (0.01) & equal (0.02) & IPOP (0.05) & csa (0.13) & 0.997508 \\
283909 & True (0.01) & False (0.06) & True (0.87) & True (0.04) & True (0.01) & False (0.09) & True (0.19) & uniform (0.42) & mirrored (0.01) & sobol (0.01) & equal (0.02) & BIPOP (0.26) & mxnes (0.28) & 0.997252 \\
415999 & True (0.02) & False (0.08) & True (0.01) & False (0.87) & False (0.02) & False (0.01) & False (0.00) & toroidal (0.37) & mirrored pairwise (0.02) & halton (0.01) & equal (0.04) & IPOP (0.09) & mxnes (0.33) & 0.997137 \\
258318 & True (0.00) & False (0.03) & True (0.07) & True (0.99) & True (0.01) & False (0.99) & False (0.02) & cotn (0.22) & nan (0.04) & sobol (0.01) & default (0.05) & IPOP (0.78) & msr (0.41) & 0.997078 \\
174006 & False (0.01) & False (0.22) & True (0.05) & True (0.85) & True (0.01) & False (0.82) & True (0.01) & mirror (0.26) & mirrored (0.06) & halton (0.01) & default (0.04) & IPOP (0.77) & csa (0.09) & 0.997077 \\
41263 & False (0.01) & False (0.02) & True (0.03) & True (0.99) & True (0.06) & False (1.00) & False (0.02) & cotn (0.41) & mirrored pairwise (0.02) & sobol (0.02) & equal (0.34) & IPOP (0.97) & msr (0.18) & 0.996977 \\
246364 & True (0.01) & False (0.08) & True (0.01) & False (0.01) & False (0.01) & True (0.01) & True (0.02) & mirror (0.38) & mirrored (0.01) & sobol (0.01) & equal (0.25) & IPOP (0.10) & mxnes (0.62) & 0.996775 \\
210328 & False (0.01) & False (0.00) & True (0.04) & True (0.05) & True (0.01) & True (0.46) & True (0.01) & uniform (0.41) & mirrored (0.04) & halton (0.01) & equal (0.15) & IPOP (0.11) & mxnes (0.59) & 0.996721 \\
53037 & False (0.02) & False (0.02) & True (0.02) & True (0.07) & True (0.01) & True (0.29) & False (0.03) & toroidal (0.44) & mirrored (0.01) & sobol (0.01) & default (0.06) & IPOP (0.32) & mxnes (0.78) & 0.996703 \\
427762 & True (0.01) & False (0.04) & True (0.02) & False (0.03) & False (0.01) & True (0.02) & False (0.02) & uniform (0.39) & mirrored (0.01) & halton (0.01) & equal (0.14) & IPOP (0.12) & mxnes (0.57) & 0.996695 \\
275380 & True (0.07) & True (0.05) & True (0.01) & True (0.10) & False (0.05) & True (0.89) & False (0.00) & toroidal (0.40) & nan (0.01) & sobol (0.01) & equal (0.01) & nan (0.01) & xnes (0.03) & 0.996616 \\
246517 & True (0.01) & False (0.03) & True (0.04) & True (0.90) & False (0.01) & False (0.93) & True (0.02) & mirror (0.38) & mirrored (0.05) & sobol (0.00) & equal (0.18) & IPOP (1.00) & msr (0.44) & 0.996567 \\
258319 & True (0.01) & False (0.08) & True (0.13) & True (0.94) & True (0.05) & False (0.99) & False (0.01) & cotn (0.20) & nan (0.04) & sobol (0.03) & equal (0.05) & IPOP (0.39) & msr (0.51) & 0.996438 \\
114433 & False (0.01) & False (0.24) & True (0.97) & True (0.39) & False (0.01) & False (0.80) & False (0.04) & cotn (0.79) & mirrored (0.46) & gaussian (0.01) & equal (0.22) & BIPOP (0.19) & xnes (0.39) & 0.996413 \\
306000 & True (0.00) & False (0.07) & True (0.14) & True (1.00) & False (0.02) & False (1.00) & True (0.01) & saturate (0.22) & mirrored (0.15) & gaussian (0.01) & default (0.04) & nan (0.70) & mxnes (0.81) & 0.996413 \\
67731 & False (0.01) & True (0.01) & False (0.01) & True (0.23) & False (0.02) & True (0.99) & False (0.10) & uniform (0.40) & nan (0.02) & sobol (0.05) & default (0.06) & IPOP (0.05) & xnes (0.11) & 0.996347 \\
22782 & False (0.16) & True (1.00) & True (0.03) & True (1.00) & True (0.01) & False (1.00) & False (0.02) & saturate (0.15) & mirrored (0.02) & sobol (0.05) & default (0.29) & IPOP (0.30) & msr (0.50) & 0.996319 \\
\bottomrule
\end{tabular}


==> cma_bias_top20_unif_original20.tex <==
\begin{tabular}{l|lllllllllllllr}
\toprule
id & active & covariance & elitist & orthogonal & sequential & threshold & sigma & bound_correction & mirrored & base_sampler & weights_option & local_restart & step_size_adaptation & unif \\
\midrule
29163 & False (0.05) & False (0.98) & True (0.97) & True (0.06) & True (0.04) & True (0.98) & False (0.07) & mirror (0.50) & mirrored pairwise (0.20) & sobol (0.22) & default (0.30) & IPOP (0.98) & tpa (0.45) & 0.980305 \\
157412 & False (0.42) & False (0.12) & False (0.98) & False (0.94) & True (0.07) & False (0.37) & True (0.00) & saturate (0.88) & nan (0.15) & halton (0.15) & 1/2^lambda (0.98) & nan (0.08) & lpxnes (0.68) & 0.979548 \\
157370 & False (0.42) & False (0.12) & False (0.98) & False (0.94) & True (0.07) & False (0.37) & False (0.00) & saturate (0.88) & nan (0.15) & halton (0.15) & 1/2^lambda (0.98) & nan (0.08) & lpxnes (0.61) & 0.979548 \\
319331 & True (0.04) & False (0.98) & True (0.98) & False (0.29) & True (0.12) & True (0.17) & True (0.14) & mirror (0.50) & mirrored pairwise (0.05) & gaussian (0.07) & 1/2^lambda (0.09) & IPOP (0.98) & csa (0.32) & 0.979526 \\
166529 & False (0.98) & True (0.98) & True (0.05) & True (0.21) & False (0.05) & True (0.98) & True (0.00) & saturate (0.83) & nan (0.10) & halton (0.18) & 1/2^lambda (0.78) & nan (0.90) & lpxnes (0.72) & 0.977983 \\
166571 & False (0.98) & True (0.98) & True (0.05) & True (0.21) & False (0.05) & True (0.98) & False (0.00) & saturate (0.83) & nan (0.10) & halton (0.18) & 1/2^lambda (0.78) & nan (0.90) & lpxnes (0.56) & 0.977983 \\
21641 & False (0.77) & True (0.98) & True (0.77) & False (0.31) & True (0.15) & True (0.09) & True (0.14) & saturate (0.94) & mirrored (0.05) & sobol (0.02) & 1/2^lambda (0.39) & nan (0.59) & psr (0.68) & 0.977025 \\
94605 & False (0.25) & True (0.98) & True (0.14) & True (0.19) & False (0.52) & True (0.69) & False (0.14) & saturate (0.97) & mirrored pairwise (0.09) & gaussian (0.15) & default (0.35) & nan (0.88) & msr (0.77) & 0.976524 \\
319341 & True (0.38) & False (0.98) & True (0.98) & False (0.06) & True (0.01) & True (0.09) & True (0.35) & mirror (0.47) & mirrored pairwise (0.04) & gaussian (0.04) & default (0.07) & IPOP (0.98) & tpa (0.38) & 0.976368 \\
269476 & True (0.07) & False (0.98) & True (0.98) & False (0.03) & False (0.04) & True (0.08) & False (0.07) & toroidal (0.43) & mirrored (0.13) & sobol (0.04) & equal (0.73) & nan (0.73) & csa (0.94) & 0.975774 \\
236600 & True (0.53) & True (0.20) & False (0.58) & False (0.25) & False (0.47) & False (0.08) & True (0.13) & saturate (0.94) & mirrored pairwise (0.47) & sobol (0.12) & 1/2^lambda (0.66) & nan (0.31) & tpa (0.44) & 0.974902 \\
167136 & False (0.84) & True (0.97) & True (0.83) & False (0.97) & True (0.09) & False (0.10) & True (0.05) & saturate (0.97) & mirrored pairwise (0.07) & halton (0.19) & default (0.30) & nan (0.96) & msr (0.84) & 0.974626 \\
21609 & False (0.93) & True (0.97) & True (0.42) & False (0.24) & True (0.15) & True (0.10) & False (0.29) & saturate (0.96) & mirrored (0.16) & sobol (0.21) & default (0.59) & nan (0.97) & msr (0.73) & 0.974452 \\
100090 & False (0.19) & False (0.97) & True (0.87) & True (0.14) & True (0.07) & True (0.97) & True (0.05) & mirror (0.47) & nan (0.08) & gaussian (0.03) & equal (0.90) & nan (0.60) & csa (0.80) & 0.973789 \\
93923 & False (0.97) & True (0.97) & True (0.42) & True (0.08) & False (0.31) & True (0.97) & False (0.03) & saturate (0.92) & nan (0.05) & gaussian (0.07) & 1/2^lambda (0.46) & nan (0.90) & psr (0.69) & 0.973618 \\
414289 & True (0.09) & False (0.97) & True (0.97) & False (0.97) & False (0.06) & False (0.23) & False (0.03) & toroidal (0.44) & nan (0.03) & halton (0.04) & equal (0.65) & nan (0.97) & csa (0.96) & 0.973343 \\
403005 & True (0.06) & False (0.97) & True (0.97) & False (0.21) & True (0.22) & True (0.15) & True (0.01) & cotn (0.80) & mirrored pairwise (0.13) & halton (0.13) & default (0.28) & nan (0.15) & tpa (0.42) & 0.973032 \\
308705 & True (0.23) & True (0.97) & False (0.97) & True (0.03) & True (0.15) & True (0.97) & False (0.14) & saturate (0.90) & nan (0.10) & gaussian (0.11) & 1/2^lambda (0.22) & nan (0.38) & csa (0.48) & 0.972774 \\
22019 & False (0.97) & True (0.97) & True (0.64) & True (0.21) & False (0.19) & True (0.97) & False (0.01) & saturate (0.94) & mirrored pairwise (0.04) & sobol (0.05) & 1/2^lambda (0.46) & nan (0.92) & psr (0.63) & 0.972674 \\
391504 & True (0.07) & False (0.83) & True (0.97) & False (0.08) & False (0.05) & True (0.04) & True (0.03) & mirror (0.44) & mirrored (0.03) & halton (0.15) & equal (0.11) & IPOP (0.97) & msr (0.70) & 0.972369 \\
\bottomrule
\end{tabular}

